Learning Semantic Role Labeling from Compatible Label Sequences

Semantic role labeling (SRL) has multiple disjoint label sets, e.g., VerbNet and PropBank. Creating these datasets is challenging, therefore a natural question is how to use each one to help the other. Prior work has shown that cross-task interaction helps, but only explored multitask learning so far. A common issue with multi-task setup is that argument sequences are still separately decoded, running the risk of generating structurally inconsistent label sequences (as per lexicons like Semlink). In this paper, we eliminate such issue with a framework that jointly models VerbNet and PropBank labels as one sequence. In this setup, we show that enforcing Semlink constraints during decoding constantly improves the overall F1. With special input constructions, our joint model infers VerbNet arguments from given PropBank arguments with over 99 F1. For learning, we propose a constrained marginal model that learns with knowledge defined in Semlink to further benefit from the large amounts of PropBank-only data. On the joint benchmark based on CoNLL05, our models achieve state-of-the-art F1's, outperforming the prior best in-domain model by 3.5 (VerbNet) and 0.8 (PropBank). For out-of-domain generalization, our models surpass the prior best by 3.4 (VerbNet) and 0.2 (PropBank).

==> conclusions.tex <==

% \section{Conclusions}
% In this work, we presented a model that learns from compatible label sequences for the SRL task.
% The proposal includes a joint CRF design, extension for learning from partially labeled data, and reasoning and learning with \Semlink constraints.
% On the VerbNet and PropBank benchmark based on CoNLL05, our models achieved state-of-the-art performance with especially strong out-of-domain generalization.
% For the newly proposed task of completing VerbNet arguments given PropBank labels, our models are near perfect, achieving over 99\% F1 scores.
